Great Models Think Alike: Improving Model Reliability via Inter-Model Latent Agreement

Reliable application of machine learning is of primary importance to the practical deployment of deep learning methods. A fundamental challenge is that models are often unreliable due to overconfidence. In this paper, we estimate a model's reliability by measuring \emph{the agreement between its latent space, and the latent space of a foundation model}. However, it is challenging to measure the agreement between two different latent spaces due to their incoherence, \eg, arbitrary rotations and different dimensionality. To overcome this incoherence issue, we design a \emph{neighborhood agreement measure} between latent spaces and find that this agreement is surprisingly well-correlated with the reliability of a model's predictions. Further, we show that fusing neighborhood agreement into a model's predictive confidence in a post-hoc way significantly improves its reliability. Theoretical analysis and extensive experiments on failure detection across various datasets verify the effectiveness of our method on both in-distribution and out-of-distribution settings.

==> dfn.tex <==
\newtheorem{observation}{Observation}
\newtheorem{conjecture}{Conjecture}
\newtheorem{problem}{Problem}
\newtheorem{algo}{Algorithm}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{question}{Question}
\newtheorem{example}{Example}
\newtheorem{answer}{Answer}
\newtheorem{proof}{Proof}

\newcommand{\hide}[1]{}
\newcommand{\notice}[1]{{\textsf{\textcolor{green}{{\em [#1]}}}}}
\newcommand{\reminder}[1]{{\textsf{\textcolor{red}{[#1]}}}}
\newcommand{\new}[1]{ {\color{blue} {#1} } }
\renewcommand{\new}[1]{ {#1} }


\newcommand{\vectornorm}[1]{\left|\left|#1\right|\right|}


\newcommand{\mkclean}{
    \renewcommand{\reminder}{\hide}
}

\newcommand{\bit}{\begin{compactitem}}
\newcommand{\eit}{\end{compactitem}}
\newcommand{\ben}{\begin{compactenum}}
\newcommand{\een}{\end{compactenum}}

\newcommand{\QED}{ \hfill {\bf QED}}
\newcommand{\method}{\textsc{OurMETHOD}\xspace}


\newcommand{\mapreduce}{\textsc{MapReduce}\xspace}
\newcommand{\hadoop}{\textsc{Hadoop}\xspace}
\newcommand{\nodeiterator}{\textsc{NodeIterator}\xspace}
\newcommand{\edgeiterator}{\textsc{EdgeIterator}\xspace}
\newcommand{\eigen}{\textsc{EigenTriangle}\xspace}
\newcommand{\dcube}{\textsc{D-Cube}\xspace}



\newcounter{definition}

\newenvironment{definition}{
	\begin{lrbox}{\coloredbgbox}
		\begin{minipage}{\dimexpr1\linewidth-2\fboxsep-2\fboxrule\relax}
			\refstepcounter{definition}
			\textbf{\textsc{Definition}.}
		}
		{
		\end{minipage}
	\end{lrbox}
	\begin{center}
		\fcolorbox{black!25}{black!03}{\usebox{\coloredbgbox}}
	\end{center}
}

 \newcounter{problem}

\newenvironment{problem}{
	\begin{lrbox}{\coloredbgbox}
		\begin{minipage}{\dimexpr1\linewidth-2\fboxsep-2\fboxrule\relax}
			\refstepcounter{problem}
			\textbf{\textsc{Problem} \theproblem.}
		}
		{
		\end{minipage}
	\end{lrbox}
	\begin{center}
		\fcolorbox{black}{black!06}{\usebox{\coloredbgbox}}
	\end{center}
}

     \newcounter{observation}

\newenvironment{observation}{
	\begin{lrbox}{\coloredbgbox}
		\begin{minipage}{\dimexpr1\linewidth-2\fboxsep-2\fboxrule\relax}
			\refstepcounter{observation}
			\textbf{\textsc{Observation} \theobservation.}
		}
		{
		\end{minipage}
	\end{lrbox}
	\begin{center}
		\fcolorbox{black!30}{black!02}{\usebox{\coloredbgbox}}
	\end{center}
}

